The maximum number of faces of the Minkowski sum of two convex polytopes

We derive tight expressions for the maximum number of $k$-faces, $0\le{}k\le{}d-1$, of the Minkowski sum, $P_1\oplus{}P_2$, of two $d$-dimensional convex polytopes $P_1$ and $P_2$, as a function of the number of vertices of the polytopes. For even dimensions $d\ge{}2$, the maximum values are attained when $P_1$ and $P_2$ are cyclic $d$-polytopes with disjoint vertex sets. For odd dimensions $d\ge{}3$, the maximum values are attained when $P_1$ and $P_2$ are $\lfloor\frac{d}{2}\rfloor$-neighborly $d$-polytopes, whose vertex sets are chosen appropriately from two distinct $d$-dimensional moment-like curves.

==> fig/shellings/coordinates.tex <==
\path (0,5.5) coordinate (y_2);
\path (0,-0.6) coordinate (y_1);

\path (1,3.8) coordinate (b_1);
\path (2,4.2) coordinate (b_2);
\path (2.3,4.6) coordinate (b_3);
\path (1.2,4.8) coordinate (b_4);
\path (0.1,4.9) coordinate (b_5); 
\path (-1.8,4.6) coordinate (b_6);
\path (-1.3,3.9) coordinate (b_7);
\path (-0.1,3.7) coordinate (b_8); 

\path (0.1,0.1) coordinate (a_1);
\path (1.5,0.4) coordinate (a_2);
\path (1.8,1.1) coordinate (a_3);
\path (0.9,1.5) coordinate (a_4);
\path (-0.1,1.7) coordinate (a_5);
\path (-1.4,1.6) coordinate (a_6); 
\path (-2.5,1.1) coordinate (a_7);
\path (-2,0.5) coordinate (a_8);
\path (-1,0.2) coordinate (a_9); % this is v


